Weighted Positive Binary Decision Diagrams for Exact Probabilistic Inference

Recent work on weighted model counting has been very successfully applied to the problem of probabilistic inference in Bayesian networks. The probability distribution is encoded into a Boolean normal form and compiled to a target language, in order to represent local structure expressed among conditional probabilities more efficiently. We show that further improvements are possible, by exploiting the knowledge that is lost during the encoding phase and incorporating it into a compiler inspired by Satisfiability Modulo Theories. Constraints among variables are used as a background theory, which allows us to optimize the Shannon decomposition. We propose a new language, called Weighted Positive Binary Decision Diagrams, that reduces the cost of probabilistic inference by using this decomposition variant to induce an arithmetic circuit of reduced size.

==> Makefile <==
# ------------------------------------------------------------------------------
# Set main file to compile
# ------------------------------------------------------------------------------

TEXFILE = paper.tex

# ------------------------------------------------------------------------------
# Determine main file to compile
# ------------------------------------------------------------------------------

ifeq ($(TEXFILE),)
    TEXFILE = $(shell find . -mindepth 1 -maxdepth 1 -type f -name "*.tex" -printf '%P ' \
		| xargs grep -r -H "documentclass" \
		| cut -d: -f1)
    MATCHES = $(shell echo $(TEXFILE) | wc -w)

    ifeq ($(shell test $(MATCHES) -eq 1; echo $$?),0)
        TEXFILE := $(basename $(TEXFILE))
    else
        $(error Cannot determine main file to compile ($(MATCHES) eligibles). Set variable 'TEXFILE' explicitly.)
    endif
else
    ifneq ($(shell test -f $(TEXFILE); echo $$?),0)
        $(error Specified TEXFILE ('$(TEXFILE)') does not exist)
    endif
endif

# ------------------------------------------------------------------------------
# Functions
# ------------------------------------------------------------------------------

recursive_wildcard=$(wildcard $1$2) $(foreach d,$(wildcard $1*),$(call recursive_wildcard,$d/,$2))
wildcarddir=$(shell find $1 -mindepth 1 -maxdepth 1 -type d 2>/dev/null)

# ------------------------------------------------------------------------------
# Environment
# ------------------------------------------------------------------------------

MAIN     = $(basename $(TEXFILE))
SHELL    = /bin/bash

DIR  	 = $(patsubst %/,%,$(dir $(abspath $(lastword $(MAKEFILE_LIST)))))
BUILDDIR = $(DIR)/build

BIB      = $(DIR)/bib
STYLE    = $(DIR)/style
PLOTS    = $(DIR)/plots
TABLES   = $(DIR)/tables
FIGURES  = $(DIR)/figures
PACKAGE  = $(DIR)/packages
DIAGRAMS = $(DIR)/diagrams
SECTIONS = $(DIR)/sections
STYLES   = $(STYLE) $(call wildcarddir,$(STYLE))
PACKAGES = $(PACKAGE) $(call wildcarddir,$(PACKAGE))

INCLUDE  = $(DIR) $(BIB) $(PLOTS) $(TABLES) $(FIGURES) $(DIAGRAMS) $(SECTIONS) $(STYLES) $(PACKAGES) $(LATEX_INCLUDE_PATH)
override LATEX_INCLUDE_PATH := $(subst $(subst ,, ),:,$(strip $(INCLUDE)))

TEXFLAGS  = -halt-on-error -file-line-error -interaction=nonstopmode -output-directory="$(BUILDDIR)"
LATEX 	  = TEXINPUTS="$(LATEX_INCLUDE_PATH):$$TEXINPUTS" pdflatex $(TEXFLAGS)
IBIBS     = $(wildcard $(DIR)/bib/*.bib) $(wildcard $(DIR)/*.bib)
OBIBS     = $(addprefix $(BUILDDIR)/, $(notdir $(IBIBS)))
BIBTEX    = bibtex
PDFVIEWER = mupdf
BIBTOOL   = bibtool -s -d -x

# ------------------------------------------------------------------------------
# Rules
# ------------------------------------------------------------------------------

.PHONY: $(MAIN) clean pdf bib plots diagrams view all

$(MAIN): pdf

pdf: $(MAIN).pdf

cite: $(BUILDDIR)/$(MAIN).bbl $(OBIBS) | $(BUILDDIR)

all:
	$(MAKE) pdf
	$(MAKE) cite
	$(MAKE) pdf
	$(MAKE) pdf

bib: force $(filter-out %references.bib,$(IBIBS)) | $(BIB)
	@$(BIBTOOL) $(BUILDDIR)/$(MAIN).aux $(IBIBS) 2>/dev/null > $(BIB)/references.bib
	@echo "references.bib created.."

$(MAIN).pdf: $(BUILDDIR)/$(MAIN).pdf
	@cp $(BUILDDIR)/$(MAIN).pdf $(DIR)/

$(BUILDDIR)/$(MAIN).pdf: force | $(BUILDDIR)
	@$(LATEX) $(DIR)/$(MAIN).tex

$(BUILDDIR)/$(MAIN).aux: pdf

$(foreach bibfile,$(IBIBS),$(eval $(addprefix $(BUILDDIR)/,$(notdir $(bibfile))): $(bibfile);	@cp $$< $$@))

$(BUILDDIR)/$(MAIN).bbl: force $(OBIBS) | $(BUILDDIR)
	@cd $(BUILDDIR); $(BIBTEX) $(MAIN);

$(BUILDDIR):
	@mkdir -p "$(BUILDDIR)"

$(BIB):
	@mkdir -p "$(BIB)"

plots: PLOTS = $(call recursive_wildcard,$(DIR)/plots,*.tex)
plots:
	sed -i 's:\\begin{tikzpicture}\[gnuplot\]:\\begin{tikzpicture}[gnuplot,scale=\\tikzscale]:g' $(PLOTS)

diagrams: DIAGRAMS = $(call recursive_wildcard,$(DIR)/diagrams,*.tex)
diagrams:
	sed -i 's:\\ensuremath{\\backslash}:\\:g' $(DIAGRAMS)
	sed -i 's:\\begin{tikzpicture}:\\begin{tikzpicture}[scale=\\tikzscale]:g' $(DIAGRAMS)

clean:
	@rm -rf "$(BUILDDIR)"

ifeq ($(firstword $(MAKECMDGOALS)),view)
ARGS := $(wordlist 2,$(words $(MAKECMDGOALS)),$(MAKECMDGOALS))
$(eval $(ARGS):;@:)
endif

view: VIEWER = $(firstword $(ARGS))
view:
	@PDFVIEWER=$$([ -z "$(VIEWER)" ] && echo $(PDFVIEWER) || echo $(VIEWER)); \
	if [ $$(command -v $$PDFVIEWER) ]; then                                   \
		echo "$$PDFVIEWER $(MAIN).pdf";                                       \
		env -i DISPLAY=$$DISPLAY $$PDFVIEWER $(DIR)/$(MAIN).pdf;              \
	else                                                                      \
		echo "Cannot view $(MAIN).pdf, Command '$$PDFVIEWER' does not exist." 1>&2;   \
		exit 0;                                                               \
	fi;

update:
	@if [ -d "$(PACKAGEDIR)" ]; then 	\
		texhash $(PACKAGEDIR);          \
	fi;
	@if [ -d "$(STYLEDIR)" ]; then      \
		texhash $(STYLEDIR);			\
	fi;

force: ;

help:
	@echo "Usage:"
	@echo "    make [option] [LATEX_INCLUDE_PATH=PATH1[:PATH2[:..]]]"
	@echo ""
	@echo "Options:"
	@echo "    pdf*          : create pdf from '$(TEXFILE)'"
	@echo "    all           : create pdf and bibtex citations"
	@echo "    bib           : create bib file"
	@echo "    cite          : bibtex citations"
	@echo "    clean         : remove latex build files"
	@echo "    update        : update local texhash"
	@echo "    view [viewer] : open pdf with [viewer]"
	@echo ""
	@echo "    * = default"
	@echo ""
	@echo "Directory hierarchy:"
	@echo "    packages : local package directory"
	@echo "    style    : local documentclass style directory"
	@echo "    build    : latex build files"



==> packages/natbib/README <==
                                 What is NATBIB?
                                 
It is a LaTeX (2e, with some support for 2.09) package to act as generalized
interface for standard and non-standard bibliographic style files (BibTeX).

It is intended primarily to produce author-year style citations from a variety
of non-standard .bst outputs; it therefore replaces the special and individual
packages that go along with such .bst files:
   apalike.sty    for    apalike.bst et al.
   newapa.sty            newapa.bst, 
   chicago.sty           chicago.bst, named.bst et al.
   harvard.sty           agsm.bst, dcu.bst, kluwer.bst et al.
   astron.sty            astron.bst, apa.bst, humanbio.bst, et al.
   authordate<n>.sty     authordate<n>.bst, aaai-named.bst
   
The above .bst files may also be used with natbib to produce author-year or 
numerical citations, so that switching from author-year to numerical is only 
a matter of selecting an option. 

The standard .bst files (plain et al) and other numerical citation .bst files
are also understood, but they can produce only numerical citations.
Replacement .bst files
   plainnat.bst
   abbrvnat.bst
   unsrtnat.bst
are provided to produce the same formatting of the reference list as the
standard equivalent, but allowing both author-year and numerical citations.

See my parallel custom-bib system for generating customized bst files.

For installation instructions and more details, see README.vxx.

Patrick W. Daly
Max-Planck-Institut f\"ur Sonnensystemforschung
D-37191 Katlenburg-Lindau, Germany
E-mail: daly@mps.mpg.de


==> sections/encoding.tex <==
\section{Encoding Bayesian Networks}\label{sec:encoding}
In order to exploit local structure, we encode BNs into \emph{conjunctive normal form} (CNF), which is the most common representation used in satisfiability solving. It consists of the conjunction of clauses, where each clause is a disjunction of literals. A literal is a propositional Boolean variable or its negation. A Bayesian Network $\mathcal{B}$ defined over variables $X$ can be seen as a multi-linear function $f : X \rightarrow \mathbb{R}$. Using a weighted adaptation of the \emph{sparse} or \emph{direct} encoding \cite{walsh2000sat,hoos1999sat}, we encode $f$ into a Boolean function $\mathcal{E}(f) = f^{e}$ by representing it as a weighted CNF:

\begin{equation}
    \mathcal{E}(f) = f^c \land f^m,
\end{equation}

where constraint clauses $f^c$ support the mapping $\mathcal{M}(f) = f^m$, that encodes probabilities and introduces a Boolean variable for each unique variable-value pair.


\subsection{Encoding Constraints}

The mapping function $\mathcal{M}$ introduces for each $x \in X$ atoms $\mathcal{A}(x) = \{x_1,\dotsc,x_n\}$, where $x_i$ signifies $x$ being equal to its $i^{th}$ value. To maintain consistency among variables we add to $f^c$ an \emph{at-least-once} (ALO) constraint clause for each $x$, to ensure $x$ is assigned a value:
\begin{equation}\label{eq:variables}
    (x_1 \lor \dotsc \lor x_n)
\end{equation}
To prohibit assigning multiple values to $x$, we add to $f^c$ the following \emph{at-most-once} (AMO) constraint clauses:

\begin{equation}\label{eq:constraints}
    \bigwedge_{i = 1}^{n}\ \ \left(x_i \implies \bigwedge_{x_j\in \mathcal{A}(x)/x_i} \overline{x_j}\right)\ \ =\ \ \bigwedge_{i = 1}^{n}\ \ \bigwedge_{j = i + 1}^{n}\ \ (\overline{x_i} \lor \overline{x_j}).
\end{equation}

\subsection{Encoding CPTs}


The factored form of the BN is preserved by using the weighted adaptation of the \emph{direct} encoding. The mapping function $\mathcal{M}$ adds a clause for every probability $P(x|U)$, where $x$ depends on variables $U = \{u^1,\dotsc,u^r\}$:
\begin{equation}\label{eq:probabilities}
        \underbrace{(\overline{\vphantom{u^1}x} \lor \overline{\vphantom{u^1}u^1} \lor \dotsc \lor \overline{\vphantom{u^1}u^r})}_{\omega_i},\\
\end{equation}
\noindent which is the logical equivalent of $(x \land u^1 \land \dotsc \land u^r \Rightarrow \omega_i)$, with symbolic weight $\omega_i$, representing probability $P(x|U)$. We introduce a $\omega_i$ for every unique probability per CPT, and thus allow multiple models to be associated with it:

\begin{equation}\label{eq:csi}
    \underbrace{\ {\strut}I^1 \land \dotsc \land I^s}_{\omega_i},\\
\end{equation}
where each $I^j$ has weight $\omega_i$ and forms the \emph{implicate} of model $m$ associated with $P(\boldsymbol{x}|\textbf{\textit{U}})$, i.e., $I^j = (\boldsymbol{x} \land \boldsymbol{u^{1}} \land \dotsc \land \boldsymbol{u^r})$, where the variables $\boldsymbol{x} \cup \textbf{\textit{U}}$ have been appropriately mapped by $\mathcal{M}$, i.e., $\boldsymbol{x} \in \mathcal{A}(x)$ and each $\boldsymbol{u^k} \in \mathcal{A}(u^k)$.


\begin{example}\label{ex:encoding}
Assume a BN as given in Example~\ref{ex:full}. The following clauses form $f^c$:
\begin{center}
    \begin{normalsize}
        \begin{tabular}{c |c| c}
            Variable & ALO (Eq.~\ref{eq:variables}) & AMO (Eq.~\ref{eq:constraints})\\\hline
            &\\[-2ex]
            $a$ & $(a_1 \lor a_2)$ & $(\overline{a_1} \lor \overline{a_2})$ \\
            $b$ & $(b_1 \lor b_2 \lor b_3)$ & $(\overline{b_1} \lor \overline{b_2}) \land (\overline{b_1} \lor \overline{b_3}) \land (\overline{b_2} \lor \overline{b_3})$\\
    \end{tabular}
    \end{normalsize}
\end{center}
The variables that make up the search space during compilation therefore are $\{a_1,a_2,b_1,b_2,b_3\}$. To encode the probabilities we identify equal $P(x|U)$:

\begin{figure}[H]
    \centering
    \begin{minipage}{0.15\textwidth}
        \centering
        \begin{normalsize}
            \setlength{\tabcolsep}{4pt}
            \begin{tabular}[t]{c | c}
                $P(a_1)$ & $P(a_2)$ \\\hline
                &\\[-2ex]
                $\omega_1$ & $\omega_1$\\
            \end{tabular}
        \end{normalsize}

    \end{minipage}
    \hspace{1em}
    \begin{minipage}{0.30\textwidth}
        \centering
        \begin{normalsize}
            \begin{tabular}[t]{c || c | c | c }
                \setlength{\tabcolsep}{2pt}
                $a$ & $P(b_1 | a)$ & $P(b_2 | a)$ & $P(b_3 | a)$\\\hline
                &&&\\[-2ex]
                1 & $\omega_2$ & $\omega_2$ & $\omega_3$\\
                2 & $\omega_2$ & $\omega_2$ & $\omega_3$\\
            \end{tabular}
        \end{normalsize}
    \end{minipage}
\end{figure}

\noindent In accordance with Equations~\ref{eq:probabilities} and \ref{eq:csi}, $f^m$ consists of the following clauses:
\begin{normalsize}
    \begin{equation}
        \nonumber
        \underbrace{(\overline{a_1})}_{\omega_1}\ \land
        \ \underbrace{(\overline{a_2})}_{\omega_1}\ \land
        \ \underbrace{(\overline{\vphantom{b_3}a_1} \lor \overline{b_1})}_{\omega_2}\ \land
        \ \underbrace{(\overline{\vphantom{b_3}a_1} \lor \overline{b_2})}_{\omega_2}\ \land
        \ \underbrace{(\overline{\vphantom{b_3}a_1} \lor \overline{b_1})}_{\omega_2}\ \land
        \ \underbrace{(\overline{\vphantom{b_3}a_1} \lor \overline{b_2})}_{\omega_2}\ \land
        \ \underbrace{(\overline{\vphantom{b_3}a_1} \lor \overline{b_3})}_{\omega_3}\ \land
        \ \underbrace{(\overline{\vphantom{b_3}a_2} \lor \overline{b_3})}_{\omega_3}
    \end{equation}
\end{normalsize}
\end{example}

Now that we have our encoding, we will take a look at the compilation process.




